Diagnosis Uncertain Models For Medical Risk Prediction

We consider a patient risk models which has access to patient features such as vital signs, lab values, and prior history but does not have access to a patient's diagnosis. For example, this occurs in a model deployed at intake time for triage purposes. We show that such `all-cause' risk models have good generalization across diagnoses but have a predictable failure mode. When the same lab/vital/history profiles can result from diagnoses with different risk profiles (e.g. E.coli vs. MRSA) the risk estimate is a probability weighted average of these two profiles. This leads to an under-estimation of risk for rare but highly risky diagnoses. We propose a fix for this problem by explicitly modeling the uncertainty in risk prediction coming from uncertainty in patient diagnoses. This gives practitioners an interpretable way to understand patient risk beyond a single risk number.

==> generic_aliases.tex <==
\RequirePackage{bbm}
\RequirePackage{mathtools}
\RequirePackage{stmaryrd}
\RequirePackage{xspace}
\RequirePackage{setspace} % for multiliner

\RequirePackage{amsfonts,amsmath,amsthm}

\newcommand{\indic}[1]{\mathbbm{1}_{\{#1\}}}
\renewcommand{\Re}{\mathbb{R}}
\newcommand{\Nat}{\mathbb{N}}
\newcommand{\expect}{\mathbb{E}}



\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}

\DeclarePairedDelimiter\intint{\llbracket}{\rrbracket}
\DeclarePairedDelimiter\norm{\lVert}{\rVert}
\DeclarePairedDelimiter\card{|}{|}
\DeclarePairedDelimiter\xset{\{}{\}}


%dot product
\DeclarePairedDelimiterX\dotp[2]{\langle}{\rangle}{#1\,\delimsize\vert\,\mathopen{}#2}

% multiliner within an equation %% FIXME for some reason it doesn't work yet
\newcommand{\multiliner}[2]{\parbox{#1}{\setstretch{1}\centering#2}}
